Towards a Client-Centered Assessment of LLM Therapists by Client Simulation

Although there is a growing belief that LLMs can be used as therapists, exploring LLMs' capabilities and inefficacy, particularly from the client's perspective, is limited. This work focuses on a client-centered assessment of LLM therapists with the involvement of simulated clients, a standard approach in clinical medical education. However, there are two challenges when applying the approach to assess LLM therapists at scale. Ethically, asking humans to frequently mimic clients and exposing them to potentially harmful LLM outputs can be risky and unsafe. Technically, it can be difficult to consistently compare the performances of different LLM therapists interacting with the same client. To this end, we adopt LLMs to simulate clients and propose ClientCAST, a client-centered approach to assessing LLM therapists by client simulation. Specifically, the simulated client is utilized to interact with LLM therapists and complete questionnaires related to the interaction. Based on the questionnaire results, we assess LLM therapists from three client-centered aspects: session outcome, therapeutic alliance, and self-reported feelings. We conduct experiments to examine the reliability of ClientCAST and use it to evaluate LLMs therapists implemented by Claude-3, GPT-3.5, LLaMA3-70B, and Mixtral 8*7B. Codes are released at https://github.com/wangjs9/ClientCAST.

==> outlet/introduction.tex <==
% Given the rising prevalence of mental and behavioral health issues \cite{gbd2022global}, the shortfall of counseling professionals \cite{rollnick2008motivational}, and the availability of LLMs, it is likely that LLMs will be increasingly used as therapists. While some users have expressed their belief that LLM therapists helped them \cite{scientificamerican2023}, some potential harms of LLM have been pointed out and perceived in real cases\cite{de2023benefits,Xiang2023}. Lacking a deep understanding of how the ``therapy outcomes'' are achieved, the utilization of LLMs as therapists could be risky and possibly harmful to their users. 

% Although previous work has attempted to assess and analyze LLM therapist behaviors from the aspect of therapist \cite{chiu2024computational}, a client-centric evaluation is lacking. 
% In addition, it cannot be assumed that evaluation from the therapist aspect is the same as the client's perceptions \cite{li2024automatic,duncan2003session,bachelor1999therapeutic}. 
% Therefore, it is essential and meaningful to investigate how clients perceive the support provided by LLMs, whether helpful or harmful.

==> tables/client_personality.tex <==
\begin{table*}[ht!]
    \centering
    \small
    \renewcommand\arraystretch{1.25}
    \begin{subtable}[t]{\textwidth}
    \centering
    \caption{Simulated Client \text{\texttimes} LLM Therapist \& Automatic Evaluation}
    \begin{tabular}{c|cc|cc|cc|cc}
    \hline
    \multirow{2}{*}{Model} & \multicolumn{2}{c|}{Problem \& Reasons for Visiting} & \multicolumn{2}{c|}{Symptoms} & \multicolumn{2}{c|}{Apparent Traits} & \multicolumn{2}{c}{Session Topic}\\
    \cline{2-9}
     & Problem Similarity & Reason Similarity & Recall & F1 & Recall & F1 & Recall & F1 \\
    \hline
    Claude-3 & 68.78\% \scriptsize{(0.71/0.22)} & \textbf{67.76\%} \scriptsize{(0.74/0.24)} & 0.77 & 0.69 & 0.71 & 0.71 & 0.84 & 0.84\\
    GPT-3.5 &  60.47\% \scriptsize{(0.64/0.25)} & 60.86\% \scriptsize{(0.66/0.26)} & 0.84 & \textbf{0.90} & 0.59 & 0.60 & 0.84 & 0.84 \\
    Llama 3-70B & \textbf{68.83\%} \scriptsize{(0.72/0.22)} & 62.29\% \scriptsize{(0.76/0.29)} & \textbf{0.86} & 0.82 & \textbf{0.78} & \textbf{0.78} & \textbf{0.88} & \textbf{0.88}\\
    Mixtral 8\text{\texttimes}7B  & 57.79\% \scriptsize{(0.74/0.34)} & 31.61\% \scriptsize{(0.81/0.56)} & 0.68 & 0.75 & 0.58 & 0.57 &  0.80 & 0.80\\
    \hline
    \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{\textwidth}
    \centering
    \caption{Simulated Client \text{\texttimes} Human Therapist \& Human Rating}
    \begin{tabular}{c|cc|cc|cc|cc}
    \hline
    \multirow{2}{*}{Model} & \multicolumn{2}{c|}{Problem \& Reasons for Visiting} & \multicolumn{2}{c|}{Symptoms} & \multicolumn{2}{c|}{Apparent Traits} & \multicolumn{2}{c}{Session Topic}\\
    \cline{2-9}
     & Problem Similarity & Reason Similarity & Recall & F1 & Recall & F1 & Recall & F1 \\
    \hline
    Claude-3 & - & - & 0.84 & 0.71 & 0.71 & 0.71 & 0.84 & 0.84\\
    GPT-3.5 &  - & - & 0.84 & 0.90 & 0.59 & 0.60 & 0.84 & 0.84 \\
    Llama 3-70B & - & - & 0.86 & 0.82 & 0.78 & 0.78 & 0.88 & 0.88\\
    Mixtral 8\text{\texttimes}7B  & - & - & 0.68 & 0.75 & 0.58 & 0.57 &  0.80 & 0.80\\
    \hline
    \end{tabular}
    \end{subtable}
    \caption{The degree to which the psychological profile is replicated by the simulated client during a new counseling session with the LLM therapist. Higher results indicate a high level of consistency in the simulated clients' behaviors. For sentence similarity, we provide the similarity value between two randomly selected sentences from the same domain after the slash for straightforward comparison.}
    \label{tab:client_simulation}
\end{table*}


INFO:root:*****claude Openness Precision: 0.73
INFO:root:*****claude Openness Recall: 0.64
INFO:root:*****claude Openness F1 Score: 0.66
INFO:root:*****claude Conscientiousness Precision: 0.79
INFO:root:*****claude Conscientiousness Recall: 0.77
INFO:root:*****claude Conscientiousness F1 Score: 0.78
INFO:root:*****claude Extraversion Precision: 0.75
INFO:root:*****claude Extraversion Recall: 0.74
INFO:root:*****claude Extraversion F1 Score: 0.73
INFO:root:*****claude Agreeableness Precision: 0.82
INFO:root:*****claude Agreeableness Recall: 0.82
INFO:root:*****claude Agreeableness F1 Score: 0.82
INFO:root:*****claude Neuroticism Precision: 0.81
INFO:root:*****claude Neuroticism Recall: 0.81
INFO:root:*****claude Neuroticism F1 Score: 0.80
INFO:root:*****claude feeling expression Precision: 0.69
INFO:root:*****claude feeling expression Recall: 0.61
INFO:root:*****claude feeling expression F1 Score: 0.62
INFO:root:*****claude emotional fluctuation Precision: 0.65
INFO:root:*****claude emotional fluctuation Recall: 0.44
INFO:root:*****claude emotional fluctuation F1 Score: 0.49
INFO:root:*****claude resistance Precision: 0.76
INFO:root:*****claude resistance Recall: 0.70
INFO:root:*****claude resistance F1 Score: 0.70

INFO:root:*********************************

INFO:root:*****gpt Openness Precision: 0.57
INFO:root:*****gpt Openness Recall: 0.55
INFO:root:*****gpt Openness F1 Score: 0.55
INFO:root:*****gpt Conscientiousness Precision: 0.65
INFO:root:*****gpt Conscientiousness Recall: 0.64
INFO:root:*****gpt Conscientiousness F1 Score: 0.64
INFO:root:*****gpt Extraversion Precision: 0.58
INFO:root:*****gpt Extraversion Recall: 0.59
INFO:root:*****gpt Extraversion F1 Score: 0.59
INFO:root:*****gpt Agreeableness Precision: 0.55
INFO:root:*****gpt Agreeableness Recall: 0.52
INFO:root:*****gpt Agreeableness F1 Score: 0.48
INFO:root:*****gpt Neuroticism Precision: 0.70
INFO:root:*****gpt Neuroticism Recall: 0.66
INFO:root:*****gpt Neuroticism F1 Score: 0.68
INFO:root:*****gpt feeling expression Precision: 0.66
INFO:root:*****gpt feeling expression Recall: 0.54
INFO:root:*****gpt feeling expression F1 Score: 0.58
INFO:root:*****gpt emotional fluctuation Precision: 0.85
INFO:root:*****gpt emotional fluctuation Recall: 0.79
INFO:root:*****gpt emotional fluctuation F1 Score: 0.82
INFO:root:*****gpt resistance Precision: 0.62
INFO:root:*****gpt resistance Recall: 0.46
INFO:root:*****gpt resistance F1 Score: 0.46
INFO:root:*********************************

INFO:root:*********************************
INFO:root:*****llama-70b Openness Precision: 0.87
INFO:root:*****llama-70b Openness Recall: 0.89
INFO:root:*****llama-70b Openness F1 Score: 0.88
INFO:root:*****llama-70b Conscientiousness Precision: 0.80
INFO:root:*****llama-70b Conscientiousness Recall: 0.79
INFO:root:*****llama-70b Conscientiousness F1 Score: 0.79
INFO:root:*****llama-70b Extraversion Precision: 0.77
INFO:root:*****llama-70b Extraversion Recall: 0.78
INFO:root:*****llama-70b Extraversion F1 Score: 0.76
INFO:root:*****llama-70b Agreeableness Precision: 0.80
INFO:root:*****llama-70b Agreeableness Recall: 0.80
INFO:root:*****llama-70b Agreeableness F1 Score: 0.80
INFO:root:*****llama-70b Neuroticism Precision: 0.77
INFO:root:*****llama-70b Neuroticism Recall: 0.77
INFO:root:*****llama-70b Neuroticism F1 Score: 0.77
INFO:root:*****llama-70b feeling expression Precision: 0.71
INFO:root:*****llama-70b feeling expression Recall: 0.71
INFO:root:*****llama-70b feeling expression F1 Score: 0.71
INFO:root:*****llama-70b emotional fluctuation Precision: 0.71
INFO:root:*****llama-70b emotional fluctuation Recall: 0.70
INFO:root:*****llama-70b emotional fluctuation F1 Score: 0.70
INFO:root:*****llama-70b resistance Precision: 0.81
INFO:root:*****llama-70b resistance Recall: 0.82
INFO:root:*****llama-70b resistance F1 Score: 0.81
INFO:root:*********************************

INFO:root:*********************************
INFO:root:*****Mixtral Openness Precision: 0.67
INFO:root:*****Mixtral Openness Recall: 0.40
INFO:root:*****Mixtral Openness F1 Score: 0.46
INFO:root:*****Mixtral Conscientiousness Precision: 0.74
INFO:root:*****Mixtral Conscientiousness Recall: 0.64
INFO:root:*****Mixtral Conscientiousness F1 Score: 0.65
INFO:root:*****Mixtral Extraversion Precision: 0.76
INFO:root:*****Mixtral Extraversion Recall: 0.77
INFO:root:*****Mixtral Extraversion F1 Score: 0.77
INFO:root:*****Mixtral Agreeableness Precision: 0.62
INFO:root:*****Mixtral Agreeableness Recall: 0.55
INFO:root:*****Mixtral Agreeableness F1 Score: 0.52
INFO:root:*****Mixtral Neuroticism Precision: 0.92
INFO:root:*****Mixtral Neuroticism Recall: 0.87
INFO:root:*****Mixtral Neuroticism F1 Score: 0.89
INFO:root:*****Mixtral feeling expression Precision: 0.54
INFO:root:*****Mixtral feeling expression Recall: 0.51
INFO:root:*****Mixtral feeling expression F1 Score: 0.52
INFO:root:*****Mixtral emotional fluctuation Precision: 0.59
INFO:root:*****Mixtral emotional fluctuation Recall: 0.48
INFO:root:*****Mixtral emotional fluctuation F1 Score: 0.47
INFO:root:*****Mixtral resistance Precision: 0.33
INFO:root:*****Mixtral resistance Recall: 0.42
INFO:root:*****Mixtral resistance F1 Score: 0.34
